Sampling lattice points in a polytope: a Bayesian biased algorithm with random updates

The set of nonnegative integer lattice points in a polytope, also known as the fiber of a linear map, makes an appearance in several applications including optimization and statistics. We address the problem of sampling from this set using three ingredients: an easy-to-compute lattice basis of the constraint matrix, a biased sampling algorithm with a Bayesian framework, and a step-wise selection method. The bias embedded in our algorithm updates sampler parameters to improve fiber discovery rate at each step chosen from previously discovered elements. We showcase the performance of the algorithm on several examples, including fibers that are out of reach for the state-of-the-art Markov bases samplers.

==> distributions.tex <==
% !TeX root = RUMBA.tex
\subsection*{Distributions}
%\sonja{Ah, this is for the appendix? what shall we do with this information.}
%{\bf \textcolor{red}{This whole section should probably be in the appendix. }}
\subsubsection*{$Y_{i,j}$ Distribution} 

(\cite{skellam1946}):
\begin{itemize}
	\item parameters: $\lambda^+,\lambda^-$
	\item support: $y\in\Z$
	\item PMF for $Y= Y^+ - Y^-$ where $Y^+ \sim \dpois(\lambda^+)$ and $Y^- \sim \dpois(\lambda^-)$: $$\pr(Y=y\mid \lambda^+,\lambda^-)=e^{-(\lambda^++\lambda^-)}\left(\frac{\lambda^+}{\lambda^-}\right)^{y/2}\Ii_y\left(2\sqrt{\lambda^+\lambda^-}\right)$$
	Where $\Ii_y$ is the modified Bessel function:
	$$\Ii_y(z)= \sum_{j=0}^{\infty}\frac{1}{j!\Gamma(j+y+1)}\left(\frac{z}{2}\right)^{2j+y}$$
	\item mean: $\Ex[Y] = \lambda^+ - \lambda^-$
	\item variance: $\Var(Y) = \lambda^+ + \lambda^-$
\end{itemize}

\subsubsection*{PMF of $X= x_t + BY$}
Given an integer matrix $A\in \Z^{N\times M}$, and a vector $u\in \Z^N$, such that $\Ff= \{x \in \Z^M \mid Ax=u\}$ is a fiber and suppose $x,x_0 \in \Ff$. Let $y \in \Z^K$ such that $x = x_0 + By$  where $B$ is a matrix of $K$ columns, spanning the lattice $\ker_{\Z}(A)$. Denote for $k\in [K]$, $Y=(Y_k)$ such that $Y_k = Y^+_k - Y^-_k$ where each $Y^+_k\sim \dpois(\lambda_k^+)$ and $Y^-\sim \dpois(\lambda_k^-)$ for some parameters $\lambda_k^+,\lambda_k^- > 0$. The PMF for $X=x$ is
\[	\pr(X=x \mid \lambda^+, \lambda^-) = \sum_{y\in \Yy_{x,x_t}}\pr(Y=y\mid \lambda^+, \lambda^-) \]
where $\Yy_{x,x_t} = \{y \in \Z^K \colon By = x- x_t\}$. If each $Y_k$ is sampled independently for $k \in [K]$, then
\[	\pr(X=x \mid \lambda^+, \lambda^-) = \sum_{y\in \Yy_{x,x_t}}\prod_{k=1}^{K}\pr(Y_k=y_k\mid \lambda^+_k, \lambda^-_k) \]
The PMF for a mixture of Poisson random variables (Skellam Distribution: \cite{skellam1946}) is
\[\pr(Y_k=y_k\mid \lambda^+_k, \lambda^-_k) = e^{-(\lambda_k^+ + \lambda_k^-)}\left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{y_k/2}\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right)\]
where $\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right)$ is the modified Bessel function:
\[\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right) = \sum_{n=0}^\infty\frac{\left(\lambda_k^+ \lambda^-_k\right)^{n+y_k/2}}{n! \Gamma(n+y_k+1)}\]
Then
\[\pr(X=x\mid \lambda^+, \lambda^-) = \sum_{y\in \Yy_{x,x_t}}\prod_{k=1}^{K} e^{-(\lambda_k^+ + \lambda_k^-)}\left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{y_k/2}\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right)\]
When $K = \text{corank}(A)$ there is a unique $y \in \Z^K$ that satisfies $By = x-x_t$. Suppose this is the case for $B$ and $y$, then
\[\pr(X=x\mid \lambda^+, \lambda^-) = \prod_{k=1}^K\pr(Y_k=y_k\mid \lambda^+_k, \lambda^-_k)\]
Denote $Y_{-k} = (Y_1,\dots, Y_{k-1}, Y_{k+1}, Y_{K})$ and $\lambda^{\pm}_{-k} = (\lambda^{\pm}_1,\dots, \lambda^{\pm}_{k-1}, \lambda^{\pm}_{k+1}, \lambda^{\pm}_{K})$  such that 
\[\pr(X=x\mid \lambda^+, \lambda^-) = \pr(Y_{-k}= y_{-k}\mid \lambda_{-k}^+,\lambda_{-k}^-)\pr(Y_k=y_k\mid \lambda^+_k, \lambda^-_k)\]
The partial derivatives of the PMF with respect to the parameters $\lambda_k^+$ and $\lambda_k^-$ for each $k \in [K]$ at $y$ are:
{\footnotesize
	\begin{align*}
		\frac{\partial\pr(X)}{\partial \lambda_k^+} 
		& = \pr(Y_{-k}= y_{-k}\mid \lambda_{-k}^+,\lambda_{-k}^-)
		e^{-(\lambda_k^++\lambda_k^-)}
		\left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{y_k/2}
		\left[
		\left(
		\frac{y_k}{\lambda_k^+}-1
		\right)\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right) + \left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{-\frac{1}{2}}\Ii_{y_k +1}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right)
		\right] \\
		\frac{\partial\pr(X)}{\partial \lambda_k^-} 
		& = \pr(Y_{-k}= y_{-k}\mid \lambda_{-k}^+,\lambda_{-k}^-)
		e^{-(\lambda_k^++\lambda_k^-)}
		\left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{y_k/2}
		\left[
		-\Ii_{y_k}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right) + \left(\frac{\lambda_k^+}{\lambda_k^-}\right)^{\frac{1}{2}}\Ii_{y_k +1}\left(2\sqrt{\lambda_k^+ \lambda_k^-}\right)
		\right]
	\end{align*}
}
